First Heuristic Then Rational: Dynamic Use of Heuristics in Language Model Reasoning

Multi-step reasoning instruction, such as chain-of-thought prompting, is widely adopted to explore better language models (LMs) performance. We report on the systematic strategy that LMs employ in such a multi-step reasoning process. Our controlled experiments reveal that LMs rely more heavily on heuristics, such as lexical overlap, in the earlier stages of reasoning, where more reasoning steps remain to reach a goal. Conversely, their reliance on heuristics decreases as LMs progress closer to the final answer through multiple reasoning steps. This suggests that LMs can backtrack only a limited number of future steps and dynamically combine heuristic strategies with rationale ones in tasks involving multi-step reasoning.

==> table/dataset/formal_language.tex <==
\begingroup
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{p{0.9\linewidth}}
        \toprule
        \textbf{Context:} \hlmelon{Peggy} has 5 apples. \hlmelon{Walter} has 2 more apples than Peggy. \hlyg{Judy}'s mother has 3 less apples than Peggy. ...\\
        \textbf{Question:} How many apples does \hlyg{Judy} have?\\
        \textbf{Reasoning Processes:} \hlmelon{Peggy} has 5 apples. \hlmelon{Walter} has 2 more apples than Peggy. ...\\
        \bottomrule
    \end{tabular}
        \caption{
    Formal language dataset with a bias to prevent the language model from outputting the shortest path. The inference process on the shortest path uses a subject different from the question.
    }
    \label{table:formal_language}
\end{table}
\endgroup
